A Symbolic Approach to Detecting Hardware Trojans Triggered by Don't Care Transitions

Due to the globalization of Integrated Circuit (IC) supply chain, hardware trojans and the attacks that can trigger them have become an important security issue. One type of hardware Trojans leverages the don't care transitions in Finite State Machines (FSMs) of hardware designs. In this paper, we present a symbolic approach to detecting don't care transitions and the hidden Trojans. Our detection approach works at both RTL and gate-level, does not require a golden design, and works in three stages. In the first stage, it explores the reachable states. In the second stage, it performs an approximate analysis to find the don't care transitions. In the third stage, it performs a state-space exploration from reachable states that have incoming don't care transitions to find behavioral discrepancies with respect to what has been observed in the first stage. We also present a pruning technique based on the reachability of FSM states. We present a methodology that leverages both RTL and gate-level for soundness and efficiency. Specifically, we show that don't care transitions must be detected at the gate-level, i.e., after synthesis has been performed, for soundness. However, under specific conditions, Trojan detection can be performed more efficiently at RTL. Evaluation of our approach on a set of benchmarks from OpenCores and TrustHub and using gate-level representation generated by two synthesis tools, Yosys and Synopsis Design Compiler (SDC), shows that our approach is both efficient (up to 10X speedup w.r.t. no pruning) and precise (0% false positives) in detecting don't care transitions and the Trojans that leverage them. Additionally, the total analysis time can achieve up to 3.40X (using Yosys) and 2.52X (SDC) speedup when synthesis preserves the FSM structure and the Trojan detection is performed at RTL.

==> DCT-explain.tex <==
\section{Case study}
\subsection{Don't-care transition detection of IMA ADPCM}
In this section, we apply our don't-care transition (DCT) detection method to the encoder part of 'IMA ADPCM' benchmark. The IMA ADPCM audio compression algorithm belongs to the Adaptive Differential Pulse Code Modulation type algorithms. The algorithm is based on a simple adaptive quantization of the difference between the input and a predictor. Each 16-bit input sample is converted to a 4-bit coded
information which yields a compression ratio of ¼\cite{IMA_ADPCM}. We will not go through detailed implementation of the design, instead, we focus on the FSM part, and especially DCTs of the FSM. 

\begin{figure*}[htbp]
\begin{center}
\includegraphics[scale=0.45]{waveform_ima_enc.png}
\caption{Simulation results of the IMA\_ADPCM encoder.}
\label{fig:ima_enc}
\end{center}
\end{figure*}

Figure \ref{fig:ima_enc} shows the simulation result of IMA\_ADPCM encoder benchmarks. The set of reachable states,  \emph{RS}, is \{000,001,010,011,100,111\} and the set of transitions, \emph{Trans}, is \{(000,000), (000,001), (001,010), (010,011), (011,100), (100,101), (101,000)\}. 

As an important aspect of our approach, a gold design is not needed.
Thus, the only thing we need to provide is a test driver as shown in Listing \ref{code:forward-code}.
To demonstrate our don't-care transition detection approach, we need to first perform forward symbolic execution to explore  state space. 
%Listing \ref{code:forward-code} shows basic workflow of forward symbolic execution code in test driver. 
We first define and declare some necessary variables such as the inputs, e.g., {\tt c0} and {\tt s0}, and the reset symbol.
The variable {\tt top} represents a pointer to the design object that represents the hardware design as implemented by Verilator.  
The circuit is reset by first enabling the reset variable and executing the design for one clock cycle (not shown). 
Then,   the reset variable gets disabled (line 7) to analyze the behavior of the circuit after the reset stage.
Inside the {\tt for loop}, the design gets executed for \emph{NUMSTEPS} clock cycles, which is set to 6 clock cycles in this case. All inputs symbolic are labeled as symbolic (lines 9-10, 12-13) for each clock cycle.
After calling the \emph{eval()} method of the design object twice, which represents one clock cycle, we restrict the state machine variable \emph{pcmSq} within the range [0,8) based on the \# of flip-flops to avoid false positives. 
Using a metadata function, {\tt klee\_add\_metadata\_globally}, that we implemented within KLEE, the current value of 
 \emph{pcmSq} is recorded in a set that is associated with a key, i.e., the address of a memory object represented by $S$, so that the set of reachable states can be computed iteratively as each symbolic path gets explored.

\begin{lstlisting}[language=c++,
                   basicstyle=\footnotesize,
                   numbers=left,
                   stepnumber=1,
                   numbersep=2 pt,
                   tabsize=4,
                   showspaces=false,
                   showstringspaces=false,
                   caption={A snippet of the forward symbolic execution step in the test-driver code.}, label=code:forward-code]
#define NUMSTEPS 6
std::set<int> S;
CData c0, c1, dest;
SData s0, s1;
Vima_adpcm_enc *top = new Vima_adpcm_enc; 
..
top->reset = 0
for(int i = 0; i < NUMSTEPS; i++){
    klee_make_symbolic(&c0, sizeof(c0),
                       "invalidFirst");
    top->inValid = c0;
    klee_make_symbolic(&s0, sizeof(s0),
                        "inSampFirst");
    top->inSamp = s0;
   
    clk = !clk;
    top->clock = clk;
    top->eval();      

    clk = !clk;
    top->clock = clk;
    top->eval();

    klee_add_metadata_globally(&S,
       top->ima_adpcm_enc->pcmSq, c0, s0);
} 
\end{lstlisting}

After performing the first stage of the analysis (lines 8-26 in Listing \ref{code:forward-code}), we perform the second stage  of the analysis, approximate symbolic execution, as shown in List \ref{code:backward-code}. 
There are two main differences between the approximate second stage and the concrete first stage. 
Firstly, in the second stage, we start from a {\em symbolic state} of the FSM instead of the reset/initial state, which means that the state variable \emph{pcmSq} could take any {\tt int} value within the range [0,8).
 %and by passing this symbolic value, source state \emph{s} can be obtained. 
 Secondly, we perform a symbolic execution of only one clock cycle rather than \emph{NUMSTEPS} clock cycles to detect the DCTs. In \emph{klee\_check\_dontcare\_transition\_globally()}, we pass \emph{st0} and \emph{pcmSq} as the source state value and the destination state value, respectively, and use the SMT solver to identify whether there is a DCT from \emph{st0} to \emph{pcmSq}, i.e., \emph{st0} $\not\in$ \emph{RS} $\wedge$ \emph{pcmSq} $\in$ \emph{RS}. 
 If so, a DCT is found and reported.

\begin{lstlisting}[language=c++,
                   basicstyle=\footnotesize,
                   numbers=right,
                   stepnumber=1,
                   numbersep=2pt,
                   tabsize=4,
                   showspaces=false,
                   showstringspaces=false,
                   caption={A snippet of code for the approximate symbolic execution part in the test-driver.}, label=code:backward-code]
klee_make_symbolic(&st0,sizeof(st0),"state");
top->ima_adpcm_enc->pcmSq = st0;	
 
klee_make_symbolic(&c1,sizeof(c1),"invalidSec");
top->inValid = c1;
   
klee_make_symbolic(&s1,sizeof(s1),"inSampSec");
top->inSamp = s1;

clk = !clk;
top->clock = clk;
top->eval();      

clk = !clk;
top->clock = clk;
top->eval();

klee_assume(top->ima_adpcm_enc->pcmSq >=0 && 
            top->ima_adpcm_enc->pcmSq < 8);
klee_check_dontcare_transition_globally(&S,top->
       ima_adpcm_enc->pcmSq, st0, dest, c1, s1);
\end{lstlisting}

Figure \ref{fig:DCT_ima_enc} shows the output of our implementation, which includes the time in seconds. We can easily find that there are two DCTs reported:  110 $\rightarrow$ 000  and 111$\rightarrow$000, which is consistent with our definition in Algirithm \ref{alg:twostage}, where both of the source states, 110 and 111, do not belong to  \emph{RS} and the destination state 000 has been recorded in \emph{RS}.


\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.45]{DCT_ima_enc.png}
\caption{Output of DCT detection for the IMA\_ADPCM decoder.}
\label{fig:DCT_ima_enc}
\end{center}
\end{figure}

\begin{table}[htbp]
\caption{Results of DCT triggered Trojan detection on IMA\_ADPCM encoder benchmark}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Transition & Output-stage 1 & Output-stage 3  & Trojan found?  \\
\hline
T(000, 000) & 0 & 1 & \cmark \\ 
%\cline{1-1}
%\cline{4-5}
T(000, 001) & 0 & 1 & \cmark\\
%\cline{1-1}
%\cline{4-5}
T(001, 010) & 0 & 1 & \cmark \\
%\cline{1-1}
%\cline{4-5}
T(010, 011) & 0 & 1 &\cmark  \\
%\cline{1-1}
%\cline{4-5}
T(011, 100) & 0 & 1 & \cmark \\
%\cline{1-1}
%\cline{4-5}
T(100, 101) & 0 & 1 & \cmark \\
%\cline{1-1}
%\cline{4-6}
T(101, 000) & 1 & 1 & \xmark\\
\hline 
\end{tabular}
\label{tab3}
\end{center}
\end{table}

\subsection{Detection of DCT triggered Trojan in IMA ADPCM}
From the simulation result in Figure \ref{fig:ima_enc}, we know that the output signal \emph{outValid} becomes high, meaning output is valid, when state machine transitions from 101 to 000. Based on this observation and the previously reported DCTs, we inserted a Trojan in the IMA ADPCM benchmark in a way that the trigger is a state machine that seeks a transition from 110 or 111 to  000 
regarding the state machine that is controlled by \emph{pcmSq}.  
Activated Trojan makes the \emph{outValid} output signal get stuck at ‘1’. 

Our DCT-triggered Trojan detection has three stages. The basic idea of the first two stages is similar to that of DCT detection except that we record additional set of observable behaviors, \emph{RBS} in  Algorithm \ref{alg:threestage}, 
like inputs, outputs, source state and destination states. 
In Listing \ref{code:trojan_detect}), variables O1 and O2 represent metadata key objects whose addresses would be used as keys to the collected metadata values during the first stage (line 1) and the third stage (line 11) in Algorithm \ref{alg:threestage}. We achieve recording additional metadata including the outputs via the {\tt klee\_add\_output\_metadata\_globally} that we added to KLEE.
Secondly, we terminate the destination states that do not have an incoming DCT to make our detection more effective. 
This is performed when don't care transitions are detected within the {\tt klee\_check\_dontcare\_transition\_globally} function as shown at lines 20-21 in Listing ref{code:backward-code}.
%Thus, in the third stage, as shown in Listing \ref{code:trojan_detect}, we start from the state that has an incoming DCT, then perform another \emph{NUMSTEPS} clock cycles forward symbolic execution 
%and record another set of \emph{RS'} (variable S' in Listing \ref{code:trojan_detect}) 
%and \emph{RBS'} (variable O2 in Listing \ref{code:trojan_detect}). 
Finally, by calling the {\tt klee\_detect\_trojan\_for\_output} function, another extension of ours, 
any deviant behavior is detected as shown at line 12 in Algorithm \ref{alg:threestage}. 

Table \ref{tab3} shows the result of DCT triggered Trojan detection on IMA\_ADPCM encoder benchmark. The first column shows various transitions in the first and third stages.
% and we only choose those transitions that have the same source states and destinations states from both stages based on Algorithm \ref{alg:threestage}. 
The next two columns represent all input conditions, there are two inputs in this case, we also need to make sure these inputs are consistent. 
Column 4 and 5 reveal output values in stage 1 and 3 respectively and the last column indicates if Trojan can be identified regarding to its transition.

It is obvious that except transition \{101\}$\rightarrow$\{000\}, all remaining transitions can reveal the Trojan, and this result is consistent with the simulation result in Figure \ref{fig:ima_enc}, where only transition 101$\rightarrow$000 can make the output signal \emph{outValid} 'high', otherwise it would stay 'low'. Thus, we know that the DCT based Trojan has been triggered and it gets the output \emph{outValid} at 'high'.
\begin{lstlisting}[language=c++,
                   basicstyle=\footnotesize,
                   numbers=right,
                   stepnumber=1,
                   numbersep=2pt,
                   tabsize=4,
                   showspaces=false,
                   showstringspaces=false,
                   caption={A snippet of Trojan detection code in the test-driver.}, label=code:trojan_detect]
// Stage 1: Forward symbolic execution
// Stage 2: Approximate symbolic execution                  
// Stage 3: Trojan Detection
// start from a state that has an incoming DCT
for(int i = 0; i < NUMSTEPS; i++){
    prevState = top->ima_adpcm_enc->pcmSq;
    // symbolize inputs
    // execute for one clock cycle
    klee_add_output_metadata_globally( &O2, 
           prevState, top->ima_adpcm_enc->pcmSq,
                    top->ima_adpcm_enc->inValid,
                     top->ima_adpcm_enc->inSamp,
          top->ima_adpcm_enc->outValid, c2, s2);
  }
  
  klee_detect_trojan_for_output(&O1, &O2);
\end{lstlisting}


